Entropy operates in non-linear semifields

We set out to demonstrate that the R\'enyi entropies with parameter $\alpha$ are better thought of as operating in a type of non-linear semiring called a positive semifield. We show how the R\'enyi's postulates lead to Pap's g-calculus where the functions carrying out the domain transformation are Renyi's information function and its inverse. In its turn, Pap's g-calculus under R\'enyi's information function transforms the set of positive reals into a family of semirings where "standard" product has been transformed into sum and "standard" sum into a power-deformed sum. Consequently, the transformed product has an inverse whence the structure is actually that of a positive semifield. Instances of this construction lead into idempotent analysis and tropical algebra as well as to less exotic structures. Furthermore, shifting the definition of the $\alpha$ parameter shows in full the intimate relation of the R\'enyi entropies to the weighted generalized power means. We conjecture that this is one of the reasons why tropical algebra procedures, like the Viterbi algorithm of dynamic programming, morphological processing, or neural networks are so successful in computational intelligence applications. But also, why there seem to exist so many procedures to deal with "information" at large.

==> Galois_connections.tex <==
%% Relators for Galois and co-Galois connections
\RequirePackage{amsmath}
\RequirePackage{fca}
%\DeclareMathOperator* \GCrel {\nearrow\hspace{-1em}\nwarrow}
%\DeclareMathOperator* \upcrossharpoons {\nearrow\hspace{-1em}\nwarrow}
\DeclareMathOperator* \GCrel {\nearrow\!\!\!\!\!\!\nwarrow}
%\DeclareMathOperator* \GCrel {\rightharpoonup\hspace{-1em}\leftharpoonup}%type0I
%\DeclareMathOperator* \coGCrel {\searrow\hspace{-1em}\swarrow}
\DeclareMathOperator* \coGCrel {\searrow\!\!\!\!\!\!\!\swarrow}
%\DeclareMathOperator* \coGCrel {\rightharpoondown\hspace{-1em}\leftharpoondown}%typeI0
\DeclareMathOperator* \multimop {\coGCrel}
\DeclareMathOperator* \GArel {\leftrightharpoons}%type00
\DeclareMathOperator* \coGArel {\rightleftharpoons}%typeII

%Some assorted symbols necessary to talk of instances of GGCC
\DeclareMathOperator\becomes{:=}% This is the symbol in language rewriting.

%%Abbreviations for types of Galois connections
\newcommand{\gctype}[1]{\textsc{type {#1}}\xspace}% Galois connectionof type...}
%\newcommand{\gctypeOI}{\textsc{type OI}\xspace}% Galois connection}
%\newcommand{\gctypeIO}{\textsc{type IO}\xspace}% Galois connection}
%\newcommand{\gctypeII}{\textsc{type II}\xspace}% Galois connection}
\newcommand{\GC}{Galois connection\xspace}
\newcommand{\GGCC}{Galois connections\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Notation for Galois connections in k-FCA
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\RequirePackage{fca}
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 
% 1. Contexts, basic concept lattices
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % 
\newcommand{\kcontext}[4][\overline{\mathcal K}]{\ensuremath{(#2,#3,\mathrel{#4})_{#1}}}
%Formal concept set\kB{\varphi}{\kcontext{\mathcal K}{G}{M}{R}}
\newcommand{\kB}[2]{\ensuremath{{\mathfrak B}^#1 #2}}
%Concept lattice%\kBV{\varphi}{\kcontext{\overline{\mathcal K}}{G}{M}{R}}
\newcommand{\kBV}[2]{\ensuremath{\BV^#1 #2}}

%These are extensions for fca.sty notation
% The concept lattices and their systems of extents and intents
\newcommand{\BVg}{\BV_G}%Alterity lattice system of extents
\newcommand{\BVm}{\BV_M}%Alterity lattice system of intents

\newcommand{\NV}{\underline{{\mathfrak N}}}%Nachbar Verband, 
\newcommand{\NL}{\NV}%Neighbourhood Lattices

% Lattices of neighbourhood of objects
\newcommand{\NVG}{\underline{{\mathfrak{N}}}}%Neighbourhood of objects  
\newcommand{\NVGg}{\NVG_G}%Neighbourhood of objects system of extents: the superindex defines the nbhood
\newcommand{\NVGm}{\NVG_M}%Neighbourhood of objects system of intents

% Lattices of neighbourhood of attributes
\newcommand{\NVM}{\underline{{\mathfrak{M}}}}%Neighbourhood of attributes
\newcommand{\NVMg}{\NVM_G}%Neighbourhood of objects system of extents: the superindex defines the nbhood
\newcommand{\NVMm}{\NVM_M}%Neighbourhood of objects system of intents

% The lattices of alterity or aliennes
\newcommand{\Aset}{\ensuremath{{{\mathfrak A}}}}
\newcommand{\AV}{\ensuremath{\underline{{\Aset}}}}%Alterity Verband, 
\newcommand{\AL}{\AV}%Alterity Lattices
\newcommand{\AVg}{\AV_G}%Alterity lattice system of extents
\newcommand{\AVm}{\AV_M}%Alterity lattice system of intents

%varphi, type of connection, semiring, G, M, R
%\newcommand{\GBV}[6][\varphi]{\ensuremath{\BV_{#2}^{#1}{\kcontext[#3]{#4}{#5}{#6}}}}
%params: varphi, type of connection, kcontext
\newcommand{\GBV}[3]{\ensuremath{\BV^{#1}_{#2}{#3}}}
\newcommand{\GNV}[3]{\ensuremath{\NV^{#1}_{#2}{#3}}}
%lattice of extents: \GBV{\varphi}{G}{\kcontext[]{G}{M}{R}}
%the lattice of intents: \GBV{\varphi}{M}{\kcontext[]{G}{M}{R}}
%[varphi], kcontext
\newcommand{\GBVOO}[2][\varphi]{\ensuremath{\GBV{#1}{\text{\textsc{oo}}}{#2}}}%Adjunction on the left
\newcommand{\GBVOI}[2][\varphi]{\ensuremath{\GBV{#1}{\text{\textsc{oi}}}{#2}}}%Galois connection
\newcommand{\GBVIO}[2][\varphi]{\ensuremath{\GBV{#1}{\text{\textsc{io}}}{#2}}}%co-Galois connection
\newcommand{\GBVII}[2][\varphi]{\ensuremath{\GBV{#1}{\text{\textsc{ii}}}{#2}}}%Adjunction on the right


%%% Names for connections used for Further Galois Connections...
%% Neighbourhood of objects
\newcommand{\NGGMI}{\ensuremath{\NVG\GMI}}
\newcommand{\NGgGMI}{\ensuremath{\NVGg \GMI}}
\newcommand{\NGmGMI}{\ensuremath{\NVGm \GMI}}
\newcommand{\NVGGMI}{\ensuremath{\NVG \GMI}}
\newcommand{\NVGgGMI}{\ensuremath{\NVGg \GMI}}
\newcommand{\NVGmGMI}{\ensuremath{\NVGm \GMI}}

%% Neighbourhood of attributes
\newcommand{\NMGMI}{\ensuremath{\NVM\GMI}}
\newcommand{\NMgGMI}{\ensuremath{\NVMg\GMI}}
\newcommand{\NMmGMI}{\ensuremath{\NVMm\GMI}}
\newcommand{\NVMGMI}{\ensuremath{\NVM\GMI}}
\newcommand{\NVMgGMI}{\ensuremath{\NVMg \GMI}}
\newcommand{\NVMmGMI}{\ensuremath{\NVMm \GMI}}

%%standard concept lattices
\newcommand{\BGGMI}{\ensuremath{{\mathfrak B}_G \GMI}}
\newcommand{\BMGMI}{\ensuremath{{\mathfrak B}_M \GMI}}
\newcommand{\BVGGMI}{\ensuremath{{\BV}_G \GMI}}
\newcommand{\BVMGMI}{\ensuremath{{\BV}_M \GMI}}

%%What about the lattice of "unrealatedness" or "alien-ness" for Extended standard FCA
\newcommand{\BAGMI}{\ensuremath{{\mathfrak B}^U \GMI}}
\newcommand{\BAGGMI}{\ensuremath{{\mathfrak B}^U_G \GMI}}
\newcommand{\BAMGMI}{\ensuremath{{\mathfrak B}^U_M \GMI}}
\newcommand{\BVAGMI}{\ensuremath{{\BV}^U \GMI}}
\newcommand{\BVAGGMI}{\ensuremath{{\BV}^U_G \GMI}}
\newcommand{\BVAMGMI}{\ensuremath{{\BV}^U_M \GMI}}

% % The following deal with SETS NOT LATTICES
\newcommand{\GCS}[3]{\ensuremath{{\mathfrak B}^{#1}_{#2}{#3}}} %Generalized concept SET not lattice.
\newcommand{\GNS}[3]{\ensuremath{{\mathfrak N}^{#1}_{#2}{#3}}} %Generalized concept SET not lattice.
\newcommand{\GNGS}[3]{\ensuremath{{\mathfrak N}^{#1}_{#2}{#3}}} %Generalized neighbourhood of obj SET not lattice.
\newcommand{\GNMS}[3]{\ensuremath{{\mathfrak N}^{#1}_{#2}{#3}}} %Generalized neighbourhood of att SET not lattice.
\newcommand{\GAS}[3]{\ensuremath{{\mathfrak A}^{#1}_{#2}{#3}}} %Generalized dual concept SET

%% Set complement operator
%\newcommand{\comp}[1]{{#1}^\complement}
\newcommand{\comp}[1]{\ensuremath{#1}^\textrm{\bf c}}

%%k extents and intents
%% remember to close the intents
%\DeclareMathOperator*  \opbigoplus {\underset{t \in T}{\stackrel{op}{\bigoplus}}}
%\DeclareMathOperator*  \opbigoplus {\stackrel{op}{\bigoplus}}
%\newcommand \opbigoplus [1]{\limits {\stackrel{op}{\bigoplus}}_{t \in T} #1}
\newcommand\kextent [1]{\sideset{_{\varphi}^{-}}{}#1}%{\left( #1\right )}}
\newcommand\kintent [1]{\sideset{}{_{\varphi}^{-}}#1}
%\newcommand\cmaxplus{\ensuremath{\overline{\mathbb R}}_{\max,+}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% ADJOINT OPERATORS FOR THE GALOIS CONNECTIONS
% VERSION 1: Follow Erné et al, 1993 in distinguishing left and right adjoints by the position of the quantifier: underscript for left adjoints, overscript for right adjoints.
% VERSION 2: Follow Cohen, quadrat, and ...., 2004 in left and right adjoints for brackets: left adjoints are notated to the right and left adjoints to the left, suggesting the direction of the arrow in the Galois Connection pair.
\RequirePackage{amsmath}
%generic left adjoint or dual adjoint param 1 is A, param 2 incidence, 3 type of connnection
%V1: \newcommand*\ladj[3]{\ensuremath{{\left( #3\right)}_{#1}^{#2}}}%
%V1.5\newcommand*\ladj[3]{\ensuremath{\sideset{}{_{#1}^{#2}}{\left( #3\right)}}}%Doesn't work because ladj is not defined as a \mathop, nor is it clear how to do so.
%V2.0
\newcommand*\ladj[3]{\ensuremath{{#3}^{#1}_{#2}}}%
%generic right adjoint or dual adjoint
%V1: \newcommand*\radj[3]{\ensuremath{{\left( #3\right)}_{#2}^{#1}}}%
%V2.0
\newcommand*\radj[3]{\ensuremath{{{}\vphantom{\protect{#3}}}^{#1}_{#2}{#3}}}%
%V4.0\newcommand*\radj[3]{\ensuremath{\smash[b]{{}\vphantom{\protect{#3}}}^{#1}_{#2}{#3}}}%
%%%%%%%%%%%%%%%%%%%% this is oh-oh or oh-aih, not zero-zero or zero-one
%% TYPE 00: one adjoint, one dual adjoint
\newcommand\ladjOO[2]{\ladj{\exists}{#1}{#2}}%
\newcommand\radjOO[2]{\radj{\forall}{#1}{#2}}%
% %%%%%%%%%%%%%%%%%%%%
% %% TYPE 0I: one adjoint, one dual adjoint
\newcommand\ladjOI[2]{\ladj{+}{#1}{#2}}%
\newcommand\radjOI[2]{\radj{+}{#1}{#2}}%
% %% TYPE I0: one adjoint, one dual adjoint
\newcommand\ladjIO[2]{\ladj{-}{#1}{#2}}%
\newcommand\radjIO[2]{\radj{-}{#1}{#2}}%
%%%%%%%%%%%%%%%%%%%%
%% TYPE II: one adjoint, one dual adjoint
\newcommand\ladjII[2]{\ladj{\forall}{#1}{#2}}%
\newcommand\radjII[2]{\radj{\exists}{#1}{#2}}%

% % % % % % % % % polars and adjuncts after LAforFCA
% TYPE 0I: with arrows in the manner of standard FCA
\newcommand{\extentOI}[2]{\ladj{\downarrow}{#1}{#2}}
\newcommand{\intentOI}[2]{\ladj{\uparrow}{#1}{#2}}
%TYPE 00: With \exists for the left and \forall for the right adjunct function.
\newcommand{\extentOO}[2]{\ladj{\forall}{#1}{#2}} %an alias for ladjOO
\newcommand{\intentOO}[2]{\ladj{\exists}{#1}{#2}} %an alias for radj00
%TYPE II: With \exists for the right and \forall for the left adjunct function.
\newcommand{\extentII}[2]{\ladj{\exists}{\transp{#1}}{#2}}
\newcommand{\intentII}[2]{\ladj{\forall}{\transp{#1}}{#2}}
% TYPE IO: with arrows in the manner of standard FCA
\newcommand{\extentIO}[2]{\ladj{\downarrow}{\linv{#1}}{#2}}
\newcommand{\intentIO}[2]{\ladj{\uparrow}{\linv{#1}}{#2}}

% Closures and operators with no notion of the underlying semifield.
\newcommand{\clextents}[2]{\ensuremath{\pi_{#1}(#2)}} %Closure of extents
\newcommand{\clintents}[2]{\ensuremath{\pi_{\transp{#1}}(#2)}} % Closure of intents.
\newcommand{\opextents}[2]{\ensuremath{\kappa_{\linv{#1}}(#2)}} % Open system of extents
\newcommand{\opintents}[2]{\ensuremath{\kappa_{\lconj{#1}}(#2)}} % Open system of intents

% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
% Notation for partitions
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
\newcommand{\parts}[1]{\ensuremath{\mathrm{Part}\!\left( #1\right)}} %Partitions of a set. %Goes to Galois_connections?
\newcommand{\kernel}[1]{\ensuremath\textrm{ker}\,#1}
% MOA does not like the OO as superindices when there are no other connections. 
\newcommand{\objconceptOO}[1]{\ensuremath{\overline{\gamma}_{\Pi}\!\!\left(#1\right)}}
\newcommand{\attconceptOO}[1]{\ensuremath{\overline{\mu}_{\Pi}\!\!\left(#1\right)}}
%\newcommand{\objconceptOO}[1]{\ensuremath{\overline{\gamma}^{oo}_{\Pi}\!\!\left(#1\right)}}
%\newcommand{\attconceptOO}[1]{\ensuremath{\overline{\mu}^{oo}_{\Pi}\!\!\left(#1\right)}}
\newcommand{\parttop}[1]{\ensuremath{\omega_{#1}}} % tops of partition lattices
\newcommand{\partbot}[1]{\ensuremath{\iota_{#1}}} % bottoms of partitions lattices.
% MOA does not like the OO as superindices when there are no other connections. 
\newcommand{\ladjobjconceptOO}[1]{\ensuremath{\overline{\gamma}_{I}\!\!\left(#1\right)}}
\newcommand{\ladjattconceptOO}[1]{\ensuremath{\overline{\mu}_{I}\!\!\left(#1\right)}}
%\newcommand{\ladjobjconceptOO}[1]{\ensuremath{\overline{\gamma}^{oo}_{I}\!\!\left(#1\right)}}
%\newcommand{\ladjattconceptOO}[1]{\ensuremath{\overline{\mu}^{oo}_{I}\!\!\left(#1\right)}}

\hyphenation{%
i-so-mor-phism i-so-mor-phisms
ho-mo-mor-phism mo-no-mor-phism anti-i-so-mor-phism%
mod-ule se-mi-mod-ule sub-se-mi-mod-ule sub-se-mi-mod-ules 
ex-per-i-ments
}


==> maxplus_minplus.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%
%%%% The following should be sent to a MAXPLUS/MINPLUS .sty
%%%%
%%%%    WARNING! This should be part of the TeX PRELUDE!!!
%%%%  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Algebraic operators for maxplus and minplus
%% Use the Moreau calculus rules for maxplus and minplus.
%% The following is a recipe from accents.tex for dealing with problems with \vec... IT works!
\RequirePackage{amsmath}
\let\vec\relax
\DeclareMathAccent{\vec}{\mathord}{letters}{"7E}
\RequirePackage{accents}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% UPPER GENERIC OPERATORS
% 0.- In this option the dots look TOO SMALL (REVIEWER'S REJECT)
%\DeclareMathOperator  \otimesu {\overset{\cdot}{\otimes}}%otimes upper
%\DeclareMathOperator  \oplusu {\overset{\cdot}{\oplus}}%otimes upper
% 1.- In this option the dots look alright.
\DeclareMathOperator  \otimesu {\overset{\centerdot}{\otimes}}%otimes upper
\DeclareMathOperator  \oplusu {\overset{\centerdot}{\oplus}}%otimes upper
\DeclareMathOperator  \odotu {\overset{\centerdot}{\odot}}%odot upper
\DeclareMathOperator  \oconvu {\overset{\centerdot}{\circledast}}%odot upper
% 2. In this option the dots look TOO BIG
%\DeclareMathOperator  \otimesu {\overset{\bullet}{\otimes}}%otimes upper
%\DeclareMathOperator  \oplusu {\overset{\bullet}{\oplus}}%otimes upper
%\DeclareMathOperator  \otimesu {\accentset{.}{\otimes}}%otimes upper
%\DeclareMathOperator  \otimesu {\overset{.}{\otimes}}%otimes upper
%%% The recipe for the next operator is from page 501. It doesn't work as a limit!
%%The following is the opposite bigoplus operator.
%% FVA: TODO. Change to {accents} notation.
\DeclareMathOperator*\opbigoplus{\underaccent{t \in T}{\stackrel{op}{\bigoplus}}}
%\DeclareMathOperator*\bigoplusl{\underset{\centerdot}{{\bigoplus}}}
%\DeclareMathOperator*\bigoplusl{\underset{\centerdot}{{\bigoplus}}}
\DeclareMathOperator*\bigoplusl{\sideset{}{_{\bullet}}\sum}
%\DeclareMathOperator*  \bigoplusu {\overset{\cdot}{\bigoplus}}%bigotimes upper
%\DeclareMathOperator*\bigoplusu{\overset{\centerdot}{{\bigoplus}}}
%\DeclareMathOperator*\bigoplusu{{\sum}^{\centerdot}}
\DeclareMathOperator*\bigoplusu{\sideset{}{^{\bullet}}\sum}
%\DeclareMathOperator*\bigoplusu{\protect{\sideset{}{^\centerdot}\Sigma}}
%The dec. above doesn'tw work because the limits are wrong!

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% LOWER GENERIC OPERATORS 
% 4.- In the next option the cdots are TOO SMALL (REJECTED BY REVIEWER'S)
%\DeclareMathOperator  \otimesl {\underaccent{\cdot}{\otimes}}%otimes lower
%\DeclareMathOperator  \oplusl {\underaccent{\cdot}{\oplus}}%otimes lower
% 1.- In the next option the centerdots are too LOW
%\DeclareMathOperator  \otimesl {\underset{\centerdot}{\otimes}}%otimes lower
%\DeclareMathOperator  \oplusl {\underset{\centerdot}{\oplus}}%otimes lower
% 2.- In the next option the centerdots are a BIT TOO SMALL
%\DeclareMathOperator  \otimesl {\underaccent{\centerdot}{\otimes}}%otimes lower
%\DeclareMathOperator  \oplusl {\underaccent{\centerdot}{\oplus}}%otimes lower
% 3.- In the next option the centerdots are too SMALL. BEST SO FAR
\DeclareMathOperator  \otimesl {\underaccent{\centerdot}{\otimes}}%otimes lower
\DeclareMathOperator  \oplusl {\underaccent{\centerdot}{\oplus}}%otimes lower
\DeclareMathOperator  \odotl {\underaccent{\centerdot}{\odot}}%odot lower
\DeclareMathOperator  \oconvl {\underaccent{\centerdot}{\circledast}}%odot upper
%5.-  In the next option the bullets are TOO BIG
%\DeclareMathOperator  \otimesl {\underaccent{\bullet}{\otimes}}%otimes lower
%\DeclareMathOperator  \oplusl {\underaccent{\bullet}{\oplus}}%otimes lower
%\DeclareMathOperator  \otimesl {\underaccent{\dot}{\otimes}}%otimes lower

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LOWER  and UPPER OPERATORS on \mathbb R
\DeclareMathOperator  \plusu {\overset{\centerdot}{+}}%plus upper
\DeclareMathOperator  \timesu {\overset{\centerdot}{\times}}%times upper
\DeclareMathOperator  \minusu {\overset{\centerdot}{--}}%plus upper
\DeclareMathOperator  \plusl {\underaccent{\centerdot}{+}}%plus lower
\DeclareMathOperator  \timesl {\underaccent{\centerdot}{\times}}%times lower
\DeclareMathOperator  \minusl {\underaccent{\centerdot}{--}}%plus upper

%% Perhaps these should be operators
\DeclareMathOperator\mpunder{\backslash}%otimes lower
%\newcommand\mpunder{\ensuremath{\backslash}}
\DeclareMathOperator\mpover{\slash}%otimes lower
%\newcommand\mpover{\ensuremath{\slash}}
%%%% LOWER RESIDUATION OPERATORS
%\DeclareMathOperator\mpunderl{\underaccent{\cdot}{\backslash}}%otimes lower
%\DeclareMathOperator\mpunderl{\underaccent{\centerdot}{\backslash}}%otimes lower
\DeclareMathOperator\mpunderl{\underaccent{\;\;\;\centerdot}{\backslash}}%otimes lower
\DeclareMathOperator\underl{\underaccent{\;\;\;\centerdot}{\backslash}}%otimes lower
%\DeclareMathOperator\mpoverl{\underaccent{\cdot}{\slash}}%otimes lower
%\DeclareMathOperator\mpoverl{\underaccent{\centerdot}{\slash}}%otimes lower
\DeclareMathOperator\mpoverl{\underaccent{\!\!\!\centerdot}{\slash}}%otimes lower
\DeclareMathOperator\overl{\underaccent{\!\!\!\centerdot}{\slash}}%otimes lower
%%%% UPPER RESIDUATION OPERATORS
%\DeclareMathOperator\mpunderu{\overset{\cdot}{\backslash}}%otimes lower
\DeclareMathOperator\mpunderu{\overset{\!\!\!\centerdot}{\backslash}}%otimes lower
\DeclareMathOperator\underu{\overset{\!\!\!\centerdot}{\backslash}}%otimes lower
%\DeclareMathOperator\mpoveru{\overset{\cdot}{\slash}}%otimes lower
\DeclareMathOperator\mpoveru{\overset{\;\;\;\centerdot}{\slash}}%otimes lower
\DeclareMathOperator\overu{\overset{\;\;\;\centerdot}{\slash}}%otimes lower

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Inf and sup convolutions: for R^n
%\DeclareMathOperator*  \supconv {\underaccent{\vee}{\circledast}}%plus lower
\DeclareMathOperator*  \supconv {\underset{\vee}{\circledast}}%plus lower
%\DeclareMathOperator*  \infconv {\underaccent{\wedge}{\circledast}}%
\DeclareMathOperator*  \infconv {\underset{\wedge}{\circledast}}%
%Min and max convolutions: for R
\DeclareMathOperator*  \maxconv {\underaccent{\max}{\circledast}}%plus lower
\DeclareMathOperator*  \minconv {\underaccent{\min}{\circledast}}%
%Name for the algebras
\newcommand{\Mmp}{max-min-plus\xspace}
\newcommand{\Maxp}{max-plus\xspace}
\newcommand{\Minp}{min-plus\xspace}

%%% Commands for Maxplus and Minplus typesetting
\newcommand\maxplus{\ensuremath{\mathbb R}_{\max,+}}
\newcommand\cmaxplus{\ensuremath{\overline{\mathbb R}}_{\max,+}}
\newcommand\minplus{\ensuremath{\mathbb R}_{\min,+}}
\newcommand\cminplus{\ensuremath{\overline{\mathbb R}}_{\min,+}}
%%% Commands for Maxtimes and Mintimes typesetting
\newcommand\maxtimes{\ensuremath{\mathbb R}_{\max,\times}}
\newcommand\cmaxtimes{\ensuremath{\overline{\mathbb R}}_{\max,\times}}
\newcommand\mintimes{\ensuremath{\mathbb R}_{\min,\times}}
\newcommand\cmintimes{\ensuremath{\overline{\mathbb R}}_{\min,\times}}
%%Completed real line
\newcommand\plustimes{\ensuremath{\overline{\mathbb R}_{+,\times}}}
\newcommand\cplustimes{\ensuremath{\mathbb R}_{+,\times}}
% Other positive semifields
\newcommand\R{\ensuremath{\mathbb R}}%just lackboard R
\newcommand\nonnegativeR{\ensuremath{\mathbb R}_0^+}%the nonnegative reals with multiplicative products
%\newcommand\nnR{\ensuremath{\mathbb R}_0^+}%An alias for the positive reals
\newcommand\nnR{\ensuremath{\mathbb R}_{\geq{0}}}%An alias for the positive reals
\newcommand\nnQ{\ensuremath{\mathbb Q}_{\geq{0}}}%An alias for the positive reals
\newcommand\nnRr[1][r]{\ensuremath{{\left (\nnR\right)_{#1}}}}%The semifields obtained by the Hölder mean transformation 
\newcommand{\hR}{\ensuremath{\mathbb H}} %Hartley semifields: simple and of order R
\newcommand\hRr[1][r]{\ensuremath{{\hR_{#1}}}}%The semifields obtained by the log-Hölder mean transformation 
\newcommand\cR{\ensuremath{{\mathbb R}_{\pm \infty}}}
%%Completed idempotent semimfield
\newcommand\cK{\ensuremath{\overline {\mathcal K}}}
\newcommand{\icK}{\ensuremath{\linv{\overline {\mathcal K}}}}
\newcommand{\dcK}{\ensuremath{\lconj{\overline {\mathcal K}}}}
%% The maxminplus or minmax algebra
%\newcommand\maxminplus{\ensuremath\overline{\mathbb R}_{\max,\min,+}}
\newcommand\maxminplus{\ensuremath\overline{\mathbb R}_{\max,\plusl}^{\min,\plusu}}
%\newcommand\maxmintimes{\ensuremath\overline{\mathbb R_0^+}_{\max,\min,\times}}
\newcommand\maxmintimes{\ensuremath\overline{\mathbb R}_{\max,\timesl}^{\min,\timesu}}
%% The positive reals and their completion
\newcommand\Rplusplustimes{\ensuremath{\mathbb R}^{+}_{+,\times}}
\newcommand\cnnRplustimes{\ensuremath{\overline{\mathbb R}}^{+}_{+,\times}}%completed nonnegative R plust times
\newcommand\Nplustimes{\ensuremath{{\mathbb N}}_{+,\times}}
\newcommand\cNplustimes{\ensuremath{\overline{\mathbb N}}_{+,\times}}

\newcommand\parmaxplus{\ensuremath{\left(\maxplus\right)}}
\newcommand\parminplus{\ensuremath{\left(\minplus \right)}}
\newcommand\parcmaxplus{\ensuremath{\left(\cmaxplus\right)}}
\newcommand\parcminplus{\ensuremath{\left(\cminplus \right)}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Different types of scalar product
%% Declaring brackets
\newcommand\bracket[2]{\ensuremath{\langle {#1}\mid{#2} \rangle}}
\newcommand\bracketdot{\ensuremath{\bracket{\cdot}{\cdot}}}
\newcommand\sqbracket[2]{\ensuremath{\left [{#1}\mid{#2} \right ]}}
\newcommand\sqbracketdot{\ensuremath{\sqbracket{\cdot}{\cdot}}}

%% Brackets with Relations in the middel
\newcommand\Rbracket[3]{\ensuremath{\langle {#1}\mid{#2}\mid{#3} \rangle}}
\newcommand\Rbracketdot[1]{\ensuremath{\Rbracket{\cdot}{#1}{\cdot}}}
\newcommand\Rsqbracket[3]{\ensuremath{\left [{#1}\mid{#2}\mid{#3} \right ]}}
\newcommand\Rsqbracketdot[1]{\ensuremath{\Rsqbracket{\cdot}{#1}{\cdot}}}

%% And ket-bras
\newcommand\ketbra[2]{\ensuremath{\rangle {#1}\mid{#2} \langle}}
\newcommand\ketbradot{\ensuremath{\ketbra{\cdot}{\cdot}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Different types of adjoints for brackets
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\RequirePackage{amssymb}
\RequirePackage{amsmath}
%\RequirePackage{galois_connections}
%left and right Galois connection adjoints (contravariant, antitone)
%\newcommand\lgc[1]{\ensuremath{#1}_\varphi^\circledast}%y_\varphi^*
%\newcommand\lgc[1]{\ensuremath{#1}_\varphi^{\_}}%y_\varphi^*
%\newcommand\lgc[1]{\ensuremath{\left( #1\right)}_\varphi^{-}}%y_\varphi^*
%Use V 2 of Galois connections adjoint functions
\newcommand\lgc[1]{\ladj{+}{\varphi}{#1}}
%\newcommand\rgc[1]{\ensuremath{}_\varphi^\circledast{#1}}%{}_\varphi^*x
%\newcommand\rgc[1]{\ensuremath{}_\varphi^{\_}{#1}}%{}_\varphi^*x
%\newcommand\rgc[1]{\ensuremath{}_\varphi^{-}{\left( #1\right)}}%{}_\varphi^*x
%\newcommand\rgc[1]{\ensuremath{}_\varphi^{-}{\left( #1\right)}}%{}_\varphi^*x
%Use V 2 of Galois connections adjoint functions
\newcommand\rgc[1]{\radj{+}{\varphi}{#1}}%{}_\varphi^*x

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% The conjugations and inversions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Left and right refer to left and right adjoints in the GC or adjunction NOT to the left and right continuous functions of the brackets.
%Right and left CGreen conjugates
%\newcommand\rconj[1]{\ensuremath{#1}^\ast}
\newcommand\lconj[1]{\ensuremath{#1}^\circledast}
%\newcommand\lconj[1]{\ensuremath{}^\ast{#1}}
\newcommand\rconj[1]{\ensuremath{\vphantom{#1}}^\circledast{#1}}
%Right and left CGQ conjugates
\newcommand\lphiconj[1]{\ensuremath{#1}_\varphi^\circledast}
\newcommand\rphiconj[1]{\ensuremath{\vphantom{#1}}_\varphi^\circledast{#1}}

%Right and left inverses
\newcommand\linv[1]{\ensuremath{#1}^{-1}}
\newcommand\rinv[1]{\ensuremath{{\vphantom{#1}}^{-1}{#1}}}
%transposes
\newcommand\transp[1]{\ensuremath{{#1}^{\textsc{t}}}}
%\newcommand\transp[1]{\ensuremath{{#1}^{\rm T}}}%too big
%\newcommand\transp[1]{\ensuremath{{#1}^{\top}}}%recalls the orthogonal adjoint

%Pseudo-inverse, aka transitive closure, and TR-closure
\newcommand\tclosure[1]{\ensuremath{{#1}^\oplus}} 
\newcommand\trclosure[1]{\ensuremath{{#1}^\circledast}}
\newcommand\tclosurel[1]{\ensuremath{{#1}^{\underaccent{\centerdot}{\oplus}}}}%otimes lower
\newcommand\trclosurel[1]{\ensuremath{{#1}^{\underaccent{\centerdot}{\circledast}}}}%otimes lower

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% The following doesn't work because sideset only applies to operators.
%\newcommand\rRgc[2]{\ensuremath\sideset{_\varphi^{#1}}{}{\left( #2\right)}}%{}_\varphi^*x
%% Commands for GGCC induced by a relation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\rRgc[2]{\ensuremath{\left( #2\right)}_\varphi^{#1}}%y_\varphi^*
\newcommand\lRgc[2]{\ensuremath{}_\varphi^{#1}{\left( #2\right)}}%{}_\varphi^*x
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Commands for completed semirings
\newcommand{\complete}[1]{\ensuremath{\overline{#1}}}
\newcommand{\completeK}{\complete{\mathcal K}}
%%%Interesting classes of K-FCA
\RequirePackage{fca}
\newcommand{\FCAabb}{FCA\xspace}
\newcommand\RmaxFCA{$\left(\maxplus \right )$-\FCA}
\newcommand\RminFCA{$\left(\minplus \right )$-\FCA}
\newcommand\cRmaxFCA{$\left(\cmaxplus \right )$-\FCA}
\newcommand\cRminFCA{$\left(\cminplus \right )$-\FCA}
\newcommand\maxminplusFCA{$\left(\maxminplus \right )$-\FCA}
\newcommand\cRmaxFCAabb{$\left(\cmaxplus \right )$-\FCAabb}
\newcommand\cRminFCAabb{$\left(\cminplus \right )$-\FCAabb}
\newcommand\maxminplusFCAabb{$\left(\maxminplus \right )$-\FCAabb}
%\newcommand\KFCA{$\left(\mathcal K\right )$-\FCA}
\newcommand\KFCA{$\mathcal K$-\FCA}
\newcommand{\KFCAabb}{$\mathcal K$-FCA\xspace}
\newcommand\cKFCA{$\overline{\mathcal K}$-\FCA}
\newcommand\GKFCA{Generalized $\mathcal K$-\FCA}
\newcommand\GFCA{Generalized \FCA}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Some hyphenation for semimodules over semirings and order morphisms
\hyphenation{%
in-fi-mum ma-xi-mum
mo-noid mo-noids di-oids di-oid 
semi-ring semi-rings  
zero-sum-free 
mo-du-loid 
mul-ti-pli-ca-tive
semi-mo-dule semi-mo-dules bi-semi-mo-dule
para-me-ter}

%%% Local Variables: 
%%% mode: plain-tex
%%% TeX-master: t
%%% End: 

